Human-Centric Research for NLP: Towards a Definition and Guiding Questions

With Human-Centric Research (HCR) we can steer research activities so that the research outcome is beneficial for human stakeholders, such as end users. But what exactly makes research human-centric? We address this question by providing a working definition and define how a research pipeline can be split into different stages in which human-centric components can be added. Additionally, we discuss existing NLP with HCR components and define a series of guiding questions, which can serve as starting points for researchers interested in exploring human-centric research approaches. We hope that this work would inspire researchers to refine the proposed definition and to pose other questions that might be meaningful for achieving HCR.

==> Human-Centric Research_ Definition & Guiding Questions - arxiv/sec-case-study.tex <==
\section{Case Study: Text Summarization}\label{sec:case-study-summarization}

\begin{table*}[h!]
\centering
\begin{tabular}{|l|m{105mm}|} 
\hline
\multicolumn{1}{|c|}{Research Stages}  & \multicolumn{1}{c|}{Guideline Questions} \\ 
\hline
HCR.1. Problem Definition & 
1.1.~What is the users' pain points and can it be solved with summarization?
1.2.~Which end user needs to read which type of text? 
1.3.~Which users' needs are not covered by the existing techniques? 
1.4.~Why do the end users need a summary?
1.5.~What do they do with the summary?
1.6.~What do they need in a summary?\\ 
\hline
HCR.2. Data Collection & 
2.1.~Does suitable data already exist or does it need to be annotated? 
2.2.~Does the annotation (summary) have to be written by the end user or can the task be outsourced to other annotators?
2.3.~What is an effective way to collect all information end users need in a summary?\\ 
\hline
HCR.3. Model building  & 
3.1.~Should the end users correct the summarization of some sentences during the training process?
3.2.~Should the end users be able to select their summarization from a series of suggested snippets?\\
\hline
HCR.4. Evaluation & 
4.1~Can we improve end users decision speed or accuracy by giving them a summary?
4.2.~How can it be determined if a summary was helpful? 
4.3.~What needs to be in a summary to address end users' pain points?
4.4.~What does the stakeholder want to do based on the summary? Can they do this with the given summary?\\ 
\hline
\end{tabular}
\caption{Guideline questions adapted as example questions for the case study of summarization.}
\label{table:usecase_summarization}
\end{table*}

For each research stage, we provided a set of guiding questions to help guide future human-centric NLP research. In particular, by adapting the provided questions for specific tasks and addressing them, researchers can explicitly state in which sense their research project is human-centric. Based on this, we provide a case study on how the task of text summarization can be enriched to be more human centric.\footnote{While ideally concrete research questions are defined by interacting with external stakeholders, the case study and adapted questions are meant to serve as starting point for researchers to explore possibilities within HCR.} For additional case studies, see the appendix.

Text summarization by itself is not necessarily a HCR task. Whether or not a summarization project is human-centric depends on the defined scope of the project. For example, the commonly used dataset CNN / Daily Mail was created because the data was easily available: it consists of news text and corresponding summary bullets \cite{nallapati-etal-2016-abstractive}. Evaluating a model trained on this dataset with humans also does not make the project human-centric if the evaluation protocol is determined by the researcher and not the external stakeholders. In contrast, \citet{hsu-tan-2021-decision} take a step in the right direction: they define their research goal as finding a summary that supports human decision making. However, they also do not involve external stakeholders as active participants in the research project. To make this research project human-centric, one could for example identify an end user group, using interview techniques inspired by design thinking methods \cite{lewrick2020design}. A research question could then be: ``\textit{How might we help [a lawyer] to [quickly understand whether a given law text will help them with their current query]?}'' We list other possible questions in Table \ref{table:usecase_summarization}.


==> Human-Centric Research_ Definition & Guiding Questions - arxiv/sec-conclusion.tex <==
\section{Conclusion}
Human-centric research (HCR) can guide research output that benefits humans and addresses their pain points. We provided a working definition of what it means to do HCR and distinguished four different research stages where HCR components can be added. %We introduced Design Thinking (DT) as a tool that can enable us to conduct HCR. 
For each research stage, we discussed existing NLP research with HCR components and formulated a series of guiding questions, which can provide a starting point for future HCR research. The Appendix provides some initial ideas on how to explore HCR for 4 different NLP tasks.  In the future we want to further develop this framework to give more concrete ideas on how the guiding questions can be addressed in a research setting. 
%We plan to develop which we would like to develop further . %and discussed how DT can help to involve relevant stakeholders to address these questions with a human-centric view.
%we discussed a series of DT principles and corresponding tools which may aid future researchers to engage with external stakeholders and to adapt a more human-centric view point in their research projects. Additionally, we provide a set of guideline questions which can be used for explicitly stating in what sense the research project is human-centric. 
%In a series of case studies, we adapt the guideline questions for particular NLP tasks to inspire future research in this direction. In its entirety, we aim to provide a good starting point for NLP researchers wanting to explore possibilities with HCR. 

==> Human-Centric Research_ Definition & Guiding Questions - arxiv/sec-definition-and-aspects-of-hc-research.tex <==
\section{Definition \& Research Stages}\label{sec:definition}
Human-centric AI (HCAI) has attracted increasing attention \cite{shneiderman2022human}, but in the broader research community it is still an open question how to best conduct HCR. Based on the definitions and essential features of HCAI discussed in recent literature, e.g., \cite{Kaluarachchi-etal-2021-review,shneiderman2020,shneiderman2022human,wu2021survey,zhu2018value,robertson2020if,holstein2019improving}, we suggest the following working definition of HCR for:

\begin{definition*}
\emph{Research is human-centric if it satisfies the following condition: human stakeholders, in addition to the researcher, actively participate in the research project.}%\footnote{For an additional discussion  see Appendix \ref{app:hcr_discussion}.}
\end{definition*}

%Intuitively human-centric research (HCR) puts the human at the center of a research project. However this alone is not sufficient to make a research project human-centric. For example, assume the following scenario: A NLP project wants to build a tool to aid school children to master a particular foreign language. This might seem a human-centric project at first. But if it does not directly involve children planning to master a foreign language, the project can not ensure that its outcome will actually be beneficial for the children. Therefore, for HCR it is important to identify the stakeholders (such as the children in the example above). These stakeholders, in addition to the researcher, should be actively involved in the research project. This directly ensures that the research outcome will have a positive benefit. 

To further clarify how stakeholders can be involved, we distinguish between four different pipeline stages within a research project:% For HCR external stakeholders have to be involved in at least one of the following stages:


\begin{itemize}

\item \textbf{Problem Definition.} The goal is to study the real needs of target users---rather than relying on the intuition of the researchers---and identify the gap between existing methods and user demands \cite{liao2020questioning,hong2021planning}. This then serves as the basis to formulate the research problem.

\item \textbf{Data Collection.} Either external stakeholders are directly involved in the data collection from planning to execution \cite{nekoto-etal-2020-participatory}, or the researchers use insights from the external stakeholders, which were obtained in the problem definition stage, to set up the data collection process. 

\item \textbf{Model Building.} There are two possible ways in which external stakeholders can impact the model building stage. (1) stakeholders may be involved before or after the training process; (2) stakeholders can be involved during model inference stage \cite{Kulesza2015, smith2018closing, Koh2017blackbox}.

\item \textbf{Task Evaluation.} 
Instead of---or in addition to---using automatic leaderboards or crowdsourced evaluations whose task is defined by researchers, systems are evaluated given requirements defined by external stakeholders \cite{ehsan2021expanding,lakkaraju2022rethinking}.
\end{itemize}

Given the definition for HCR and by distinguishing different research stages, we can discuss different opportunities and possibilities for HCR in a more structured manner.

==> Human-Centric Research_ Definition & Guiding Questions - arxiv/sec-discussion.tex <==
\section{Discussion}\label{sec-discussion}

==> Human-Centric Research_ Definition & Guiding Questions - arxiv/sec-introduction.tex <==
\section{Introduction}
Research advances are driven by curiosity and the need to improve human life. Often research addresses fundamental core challenges. Other times research is more application oriented. With the recent significant progress in NLP, the NLP community has the opportunity to address more and more application oriented research questions. However, such research is not necessarily human-centric: the research questions and the methods for answering them are often entirely designed and implemented by the researchers and their intuition. 

In contrast, Human-Centric Research (HCR) aims to ensure that \textit{human stakeholders} benefit from the outcome of the research. The stakeholders are people that have a stake in the research outcome and may include researchers,
%\footnote{We see researchers as stakeholders as they have an interest in the result and outcome of the project. Additionally they have to judge project feasibility and need to consider ethical implications from a technology point of view.} 
end users, data collectors, feedback providers or domain experts. We use the term \textit{external stakeholders} to refer to stakeholders other than the researchers. In HCR, the goal is to place \emph{all} stakeholders at the center of research, not only the researchers themselves. 
Not involving external stakeholders introduces the risk of spending great amounts of time and resources in solving problems that might turn out to be irrelevant in practical settings. With HCR, we would like to ensure that external stakeholders benefit from the outcome of the research by directly involving them in the research process.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.45,trim={5.5cm 5.3cm 5.5cm 5.3cm},clip]{figures/fig_1v13.pdf}
    \caption{Human-Centric Research (HCR) should involve stakeholders other than the researchers themselves. We define four stages in the research pipeline where other stakeholders can be involved.}
    \label{fig:dt-nlp}
    \vspace{-0.5em}
\end{figure}

Human-centric research components are used increasingly in the NLP community. For example in evaluation \cite{ribeiro-etal-2020-beyond,hong2021planning}, design \cite{park2021facilitating, wang-etal-2021-putting, iskender-etal-2021-towards} and exploration \cite{lertvittayakumjorn2021explanation,heuer-buschek-2021-methods} of NLP models in various tasks such as machine translation \cite{nekoto-etal-2020-participatory}, dialogue systems \cite{Xiao2020chatbot}, text summarization \cite{smith2018closing,hsu-tan-2021-decision,passali-etal-2021-towards}, natural language generation \cite{tintarev2016personal,clark2018creative,akoury-etal-2020-storium}, information extraction \cite{gashteovski-etal-2020-aligning} and other applications \cite{rello2015spellchecker}. 

As a community, however, we lack a clear definition of what HCR means. With a clear definition it would be easier for researchers to find more human-centric research questions and to better communicate in what way their research is human-centric. To tackle these open problems, we make the following contributions. First, we formulate a working definition for the term ''human-centric research`` and define different stages of research which can be made more human-centric (Section \ref{sec:definition}). For an overview of the research stages see Figure \ref{fig:dt-nlp}. Second, we review recent literature in the field of NLP with respect to HCR and formulate and discuss a series of guiding research questions for future HCR projects. Finally, we present one example case study that showcases how the guiding questions can be adapted for particular NLP tasks (Sec.~\ref{sec:case-study-summarization}).%This interplay between HCR, our defined research stages and DT is visualized in Figure \ref{fig:dt-nlp}. 
%Finally, we present one example case study that showcases how the guiding questions can be adapted for particular NLP tasks (Section \ref{sec:case}).


==> Human-Centric Research_ Definition & Guiding Questions - arxiv/sec-questions.tex <==
\section{Guiding Questions in Research Stages}\label{sec:stages}
%Given the definition of the different research stages, 
%We can now take a closer look at how we can make each research stage to more human-centric. For each research stage, we discuss the following two points: (1) recent literature in the field of NLP on the respective stage that aligns with the HCR paradigm; (2) guiding questions that can inspire future HCR projects.
For each research stage we now formulate a series of guiding questions that can inspire future HCR.

\subsection{Stage 1: Problem Definition}\label{sec:pd}
Many research projects are not human-centric, because they do not take into account real human needs at inception; rather, they reflect the researcher's personal intuition and interest. Previously human-centric inspired NLP problems were for example machine translation \cite{weaver} or information extraction \cite{wilks1997information}, which were either defined or driven by real human need. Recent times have seen the emergence of more human-centric NLP tasks, such as the detection of hate speech on social media \cite{basile2019semeval} or fact checking \cite{mihaylova2019semeval}. These tasks are arguably human-centric---because they solve problems inspired by real human need---yet, they still typically lack the active involvement of the human stakeholders in the problem definition. To address this gap, we formulate four blocks of guiding questions that can help to make the problem definition of a research project more human-centric.

\paragraph{Guiding Questions.} 
\begin{itemize}
    \item Selection: Which NLP task will be tackled? What methods should be used?
    \item Stakeholders: Who are the stakeholders, what are their characteristics?  Who are the end users most affected by the system? Who operates the system, who owns it? Who shall be the target stakeholder?
    \item Pain points: What are the pain points for the target stakeholder?
    \item Research question: What are the shortcomings of existing methods? What research question should we ask to address these shortcomings in a research project?
    %\item Selection: Which m
\end{itemize}
Researchers often start by choosing an NLP task of interest and identifying gaps in research, which they would be interested in addressing. Typically the research is now conducted by the researchers without any additional outside input. In contrast, in a more human-centric view, researchers could first identify and involve stakeholders to derive a problem definition that would directly benefit the stakeholders by addressing their pain points in the area of research identified by the researchers. By this early involvement, the researchers can ensure that their research can have a direct positive impact.

Once a pain point to be addressed is defined, researchers should determine how well existing technology is able to address the defined problem. For this, the researchers, as the experts of the NLP domain, should analyse (1) which NLP task is most suitable and (2) what existing methods are a good starting point to solve the problem. Regarding the task selection, the researchers need to understand the problem as described by the other stakeholders and then to match it to the most suitable NLP task. This could for example be sequence classification, token classification, sequence generation or another task. Once the task is chosen, the researchers should explore promising existing methods which can solve the task. Here it is important that the researchers consider all viable options and that they do not restrict themselves to methods that they have previously used or know well.

\subsection{Stage 2: Data Collection}\label{sec:dc}
The design of training datasets as well as systems that support data collection, are crucial for creating effective human-centric NLP systems. For example, the standard crowdsourcing procedures could be intuitively considered as human-centric, because the data is collected with human input from non-researchers. Such crowdsourcing tasks, however, are defined by the researcher. With these constraints, neither the crowdworkers nor other external stakeholders (such as end users) can express their pain points outside of the limitations imposed by the researchers. Therefore, the process lacks creative human input from non-researchers, with which more meaningful data could be collected. 

Prior work on human-centric data collection includes (1) system that facilities domain knowledge acquisition from domain experts \cite{park2021facilitating}, (2) collection process that is gamified, e.g.~by asking users to generate text in a role playing game \citep{akoury-etal-2020-storium}, or (3) systems for machine-human co-creation \cite{clark2018creative,iskender-etal-2020-towards,tintarev2016personal}. The above examples demonstrate that NLP data generation tasks can benefit from creative and human-centric implementation of the data collection stage. The setup of future human-centric data collection projects can be facilitated by the following guiding questions.

\paragraph{Guiding Questions.}
\begin{itemize}
    \item Data: What data needs to be collected to solve the pain points of the end users?
    \item Annotation: Who is qualified to annotate? 
    \item Collection Approach: How should the annotation be done?
\end{itemize}

To address the above questions, ensure that all important angles are considered as well as offer transparency w.r.t.~to the collected data for all stakeholders, we recommend the guide on creating datasheets for new datasets by \citet{datasheets}.
%we also recommend the researchers to follow the guide on creating datasheets for new datasets by \citet{datasheets}.

%The detailed questions posed by \citet{datasheets} will ensure that all important angles are considered as well as offer transparency with regards to the collected data for all stakeholders.

\subsection{Stage 3: Model Building}\label{sec:mb}
Model building includes (1) defining the model and the training process, and (2) specifying the inference strategy. Typically this is done at the prerogative of the researcher, but both components can be made more human-centric. For example, model training could involve stakeholders during or after training. Overall, the type of human-machine interaction during the model building shapes whether it is a human-in-the-loop \cite{smith2018closing, yuksel2020human, khashabi2021genie} or machine-in-the-loop~\cite{clark2018creative}. The former means the user intervenes with the system operation, and the latter happens when the system’s support is triggered by the user to finish a  task.

During inference time, humans can provide inputs to assist the model with predictions (e.g. \citet{wen2019human,rello2015spellchecker}). In the context of explainable systems, stakeholders can for example be involved to 
ensure that a model follows certain explanations \cite{zhang2016, Zaidan2007, Arous2021}. Whether either type of involvement is desired, should be addressed in a discussion with all stakeholders.

\paragraph{Guiding Questions.}
\begin{itemize}
    \item Prototype: Can the designed model fulfil the external stakeholders' expectations?
    \item Inference: Should a stakeholder be involved in the inference process of the model?
    %\item Control: Who makes the final decision, the model or a stakeholder?
\end{itemize}

To explore the answer to both questions, we recommend the researchers to repeatedly interact with the stakeholders in order to refine the prototype's architecture and to understand how end users later want to interact with the model. During the first iterations, one option could be to create simple mock-ups, e.g.~in form of slides that showcase the functionality and planned end user interaction. Once both questions can be answered sufficiently, the researchers can then start to build the system. Once a system is built and reaches an acceptable performance from the researchers' point of view, the researchers can start a continuous feedback loop between this stage and the next stage: task evaluation with the stakeholders.

\subsection{Stage 4: Task Evaluation}\label{sec:te} NLP systems are often evaluated on standard NLP benchmarks using scores averaged across a test set, such as accuracy (\textsc{GLUE} \cite{glue},  \textit{inter alia}). While such automatic benchmarking provides quick evaluation---and, consequently, speeds up NLP research---such a metric may fail to capture the diverse needs of the end users \cite{ethayarajh2020utility,narayan2021personalized}.

To address the issue of averaged metrics, \citet{ribeiro-etal-2020-beyond} propose to check systems against different types of examples. Other efforts in this direction include carrying out interviews to study NLP system failures \cite{hong2021planning} or investigating human debugging of NLP models \cite{lertvittayakumjorn2021explanation}. While these works move into the right direction, they do not explicitly capture human reactions from stakeholders, such as whether a system meets expectations or which open pain-points remain and what future wishes exist. For this, we formulate the following guiding questions.
\paragraph{Guiding Questions.}  
\begin{itemize}
    \item Metric: What is a good evaluation measure?
    \item Evaluator: Who evaluates the built model?
    \item Level: At which level is the task evaluated?
    \item Impact: What is done after the evaluation?
\end{itemize}

Especially when a human evaluator is involved, it is important to carefully investigate and define an appropriate evaluation metric (1st question). Together with external stakeholders, the researchers should determine the criteria for assessing if a stakeholder's pain point is addressed by the model. %For example, in the context of explainable AI, one could say: \emph{Given the users' pain point of wanting to understand if an AI model is correct, a suitable explanation should allow the users to correctly determine whether a prediction is true or false}. 
Once a metric is defined, all stakeholders should also address the question whether the evaluation task has been set up in a way that the evaluator can understand the task at hand. %Additionally, this also allows to determine who the appropriate evaluators are.% and whether they require any type of training before the evaluation.

With regards to the 2nd and 3rd questions, the final goal should be that a target stakeholder evaluates the model on a task that aims to address their pain point(s). However, jumping straight to this setting may not be practical in most situations. Therefore, following \citet{doshivelez2017rigorous}, we propose an overall 3-step process for evaluation: (1) \textit{Non-HCR}: perform an automatic evaluation to ensure the model output is reasonable. Since human evaluators can be a rare and/or costly resource, an automatic evaluation provides a baseline level for quality. (2) \textit{Towards HCR}: recruit a human evaluator and evaluate on a pseudo-task. Due to time and cost constraints, it is often easier to find lay users (instead of e.g. a doctor) for evaluation. Additionally, if the real task is very complex, then a pseudo-task is helpful as a stepping stone; (3) \textit{HCR}: ask the targeted stakeholder to evaluate the model built to solve their pain point(s).

%Finally, one can obtain direct insights about the users' needs. The end users interact with the trained model and 
Finally, researchers can observe or interview end users to understand if the model addresses their pain points, fulfils their needs etc. This aids to address the 4th question: the insights can be used in an iterative way to improve the model building stage. Overall, the findings from the test stage can enrich the evaluation of research projects with a new dimension: stakeholders' feedback.



==> sec-discussion.tex <==
\section{Discussion}\label{sec-discussion}
